A Declarative Framework for Specifying and Enforcing Purpose-aware Policies

Purpose is crucial for privacy protection as it makes users confident that their personal data are processed as intended. Available proposals for the specification and enforcement of purpose-aware policies are unsatisfactory for their ambiguous semantics of purposes and/or lack of support to the run-time enforcement of policies. In this paper, we propose a declarative framework based on a first-order temporal logic that allows us to give a precise semantics to purpose-aware policies and to reuse algorithms for the design of a run-time monitor enforcing purpose-aware policies. We also show the complexity of the generation and use of the monitor which, to the best of our knowledge, is the first such a result in literature on purpose-aware policies.

==> 3.0-preliminaries.tex <==
%!TEX root = ./main.tex

\section{Preliminaries}
\label{sec:preliminaries}



%%



\subsection{Process specification language}

We consider a company business \emph{processes} as \emph{purposes}
which data are accessed, and possibly modified for. Indeed, it is
natural to answer the question: ``What is the reason data are used
for?'' with: ``In order to achieve this objective''. Such an answer
exactly complies with the widely-accepted definition of business
process as: \emph{the set of activities which realize a goal}
\cite{Weske-BPMBook,Dumas-BPM-book,AalstStahl2011-book}.

From the definition of business processes as sets of activities aimed
at realizing specific goals, follows that \emph{activities} or
\emph{tasks} (from now on we will use these terms interchangeably) are
the main processes building blocks and the only that can access and
modify data. 
% Typical examples of tasks are
% $\msf{addToChart}$, $\msf{shipment}$ or $\msf{payment}$, while
% $\msf{customerAquisition}$, $\msf{hiring}$ or $\msf{orderToCash}$ can
% be considered as business goals. Conceptually, tasks are modular and
% possibly complex activities meaningful at a business level.
% Practically, we do not pose any restriction on their structure or
% complexity, as we are only interested on which data they access.
% %%
% This is in line with the recent trend in the \bpm field of considering
% very seriously the linkage between processes and data. While early
% business process models lacked the data dimension focusing on the
% activity perspective only, recent models try to bridge the gap between
% such aspects \cite{MeyerSW11}.
% %%
% Also, data can \emph{only} be accessed through tasks. This
% assumption is reasonable as, on the one hand, once the business
% objetives have been clearly and formally defined, there are no other
% reasons to access data if not for achieving them, and on the other, when
% the need of accessing data in a specific way arises, it is always
% possible to define a specific tasks for the purpose.

We use \declare for specifying business processes, a
declarative process modeling language originally introduced in
\cite{AalstPS09}.
%%
While most of the languages for specifying business processes are
based on an procedural approach \cite{Weske-BPMBook}, meaning that
they explicitly describe all the allowed sequences of tasks (or
activities), \declare specifies a set of constraints that must not be
violated during process executions.  In this way, the language enjoys
flexibility and is suitable for specifying purpose-based policies.

Technically, constraints are specified by propositional
\LTL formulas on finite execution traces where the set of
propositional symbols represent tasks.  In order to make the language
more accessible to non-technical people, among all possible \LTL
constraints, some specific ``patterns'' have been singled out as
particularly meaningful for expressing processes and associated to 
graphical symbols. Those are basically formulas templates such as
existence, precedence, succession and choice between activities.


Given a set of symbols $\P$ (in our case representing tasks) \LTL
formulas are built as follows:
%%
\[\varphi ::= a \mid \lnot \varphi \mid \varphi_1\land
\varphi_2 \mid \Next\varphi \mid \varphi_1\Until\varphi_2 \mid
\varphi_1 \Wuntil \varphi_2 \mid \Box \varphi \mid \Diamond \varphi
\text{~~~with $a\in\Prop$}\]
%%
Intuitively, $\Next\varphi$ says that $\varphi$ holds at the
\emph{next} instant; $\varphi_1\Until\varphi_2$ says that at some
future instant $\varphi_2$ will hold and \emph{until} that point
$\varphi_1$ holds; its weak version $\varphi_1 \Wuntil \varphi_2$ says
essentially the same but $\varphi_2$ can also hold forever;
$\Box \varphi$ means that $\varphi$ always holds while is dual
$\Diamond \varphi$ that $\varphi$ eventually holds.

Semantics of \LTL formulas is given in terms of executions or
\emph{traces}, representing the process temporal evolutions, i.e,
sequence of tasks. We assume processes to \emph{eventually
  terminate}. Thus, instead of using the original infinite-trace
semantics of Pnueli \cite{Pnueli77}, we adopt a finite-trace
semantics. Technically, a trace $\pi$ is a finite word over the
alphabet of $2^{\P}$, i.e, over interpretations for symbols in
$\P$. Given a finite trace $\pi$ and a \LTL formula
$\varphi$, the truth relation $\pi \models \varphi$ is inductively defined,
and we refer to \cite{DeGiacomoMGMM14,DeGiacomoDMM14} for the
technical aspects. The only notable detail of the finite-trace semantics is that
$\Next \phi$ is true iff a next state actually exists \emph{and} it
satisfies $\varphi$.
%%
% \todo[inline]{Decidere se levare.}  A formula $\varphi$ is
% \emph{satisfiable} if it is true in some finite trace, and it is
% \emph{valid} if it is true in every finite trace. A formula $\varphi$
% logically implies a formula $\varphi'$, written
% $\varphi \models \varphi'$, if for every finite trace $\pi$ we have
% that $\pi\models\varphi$ implies $\pi\models\varphi'$. Notice that
% satiability, validity and logical implication are all immediately
% mutually reducible to each other and known to be
% \textsc{pspace}-complete \cite{DeGiacomoV13,SistlaClarke1985}: for
% example $\varphi$ is valid iff $\lnot\varphi$ is
% unsatisfiable. Similarly, $\varphi \models \varphi'$ iff
% $\varphi \land\lnot\varphi'$ is unsatisfiable.
%%

% We will make use of the following abbreviations:
% \begin{compactitem}
% \item $\true$, $\false$, $\lor$, $\limp$;
% % \item $\Wnext\varphi = \lnot\Next\lnot\varphi$ is interpreted as a
% %   \emph{weak next}, stating that if $\Last$ does not hold then
% %   $\varphi$ must hold in the next state;
% \item $\Diamond\varphi = \true\Until\varphi$ says that $\varphi$ will
%   \emph{eventually} hold before the last instant (included);
% \item $\Box\varphi = \lnot\Diamond\lnot\varphi$ says that from the
%   current instant till the last instant $\varphi$ will \emph{always}
%   hold;
%   % \item
%   %   $\varphi_1 \Release \varphi_2 = \lnot(\lnot\varphi_1 \Until
%   %   \lnot\varphi_2)$
%   %   means that $\varphi_1$ \emph{releases} $\varphi_2$, i.e., either
%   %   $\varphi_2$ must hold forever, or until $\varphi_1$ also holds;
% \item
%   $\varphi_1 \Wuntil \varphi_2 = (\varphi_1 \Until \varphi_2 \lor \Box
%   \varphi_1)$
%   is interpreted as a \emph{weak until}, and means that $\varphi_1$
%   holds until $\varphi_2$ or
%   forever. %Notice that $\varphi_1 \Release \varphi_2$ can be also expressed as $\varphi_2 \Wuntil (\varphi_1\land\varphi_2)$.
% \end{compactitem}

As customary when modeling process constraints \cite{AalstPS09}, we
assume that a single task is performed at a time. This is formally
captured by implicitly assuming the additional constraint in processes specification:
$
\Box(\bigvee_{a\in\P} a) \land \Box(\bigwedge_{a,b\in\Prop, a \neq b}
a \limp \lnot b) %\land \Box(\Wnext \false \leftrightarrow \Ended)
$.
%%
Let $\varphi$ be the conjunction of constraints. In practical terms,
$\varphi$ represents the set of allowed traces (or process executions)
$\pi$, i.e, traces $\pi$ such that $\pi \models \varphi$. Such a set is
also called the \emph{language} of $\phi$ and written $L(\varphi)$.
%%
Given a formula $\varphi$ we can build an \emph{automaton}, i.e., a
finite-state machine (see
\cite{DeGiacomoMGMM14,DeGiacomoDMM14} for the actual procedure) that
accepts exactly all traces belonging to $L(\varphi)$.





\subsection{Database}

The state of the system is stored in a relational database. The
database contains the rule- and data-centric policies, which
constitute the \emph{static} part, and also keeps track of information
concerning the processes' evolutions, which, evolving over time,
represents the \emph{dynamic} part. As we will reason on policies and
their interaction with the dynamic evolution of processes, we define
the database schema $\D$ as a first-order language with equality and
no function symbols, as to express properties and check complex
queries using first-order logic.
%%
The set of first-order formulas is build as usual starting from $\D$,
from an infinite set of values and from an infinite set of constant
symbols. We require constants to be interpreted as themselves,
blurring the distinction between contants and values, and from now on
we use $\msf{sans}$ $\msf{serif}$ font for denoting them, while
$traditional$ font for predicates and variables.
%%
Constants are \emph{sorted}, namely, they have a type, hence
predicates in $\D$ range over sorts. In order to keep the dissertation
readable, we do not introduce the technical machinery needed to
formally define sorts.

A database instance for the static part of the schema $\D_{st}$ is a tuple
$I_{st}=(\Delta_{st}, \cdot^I_{st})$, where $\Delta_{st}$ is a
possibly infinite interpretation domain, and
$\cdot^I_{st}$ is an interpretation function associating each
predicate symbol $R_{st} \in \D_{st}$ of arity $n$ to a relation
$R_{st}^I \subseteq \Delta_{st}^n$.
%%
The finite subset of $\Delta_{st}$ of elements occurring in relations
is called active domain of $I_{st}$ and denoted by $adom(I_{st})$.
%%
The same definitions directly apply to the dynamic part $\D_{dy}$ as
well, with the exception of the domain that can be written as
$\Delta_{dy}=\Delta_{st} \cup \Delta_{wf}$, where $\Delta_{wf}$ is
the interpretation domain for workflow ids (see Section
\ref{subsec:Framework-database}).
%%
We denote by $I$ an interpretation of the whole schema $\D$, i.e.,
$I=I_{st} \cup I_{dy}$.

Let $\psi$ be a $\D$-formula and $I$ a $\D$-instance. We use
$I \models \psi$ for the usual first-order logic satisfaction
relation, see any standard book on logic, e.g., \cite{VanDalenBook}.









% \subsection{Constraints}



% Having a formal specification of processes, we can express
% \sod and \bod constraints, which
% enhance \rbac policies by expressing restrictions \emph{which depend
%   on the current process evolution}. Indeed, while \rbac policies are
% ``static'', e.g., ``Sam can access his job experience data'', \sod and
% \bod depend on a specific execution, namely: ``\emph{who} performes the
% $\msf{interview}$ cannot also perform $\msf{findJobs}$''. If Alice
% performed the interview, then she cannot perform job searching, but
% the interview could also have been performed by someone else.  From a
% technical viewpoint, verify such constraints involves a complex form of
% temporal reasoning. Let us assume the previous \sod constraint, that
% Alice and Bob are the only JH employees and that Bob does not have the
% \rbac privileges to access data manipulated by $\msf{findJobs}$. Then,
% if Alice requests to perform $\msf{interview}$, our 
% technique immediately discovers a process violation and blocks the
% request, as it infers that if Alice performs the interview,
% than nobody else can perform $\msf{findJobs}$ in the future, hence
% violating the $\Diamond \msf{findJobs}$ constraint.






























%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

\endinput

==> 3.2-purposeFramework.tex <==
\subsection{Purpose formalization}
\label{sec:purpose}

We resume our running example by
formalizing the $\msf{jobHunting}$ process.


\begin{example}
Each bullet is a constraint and the set of formulas' atomic
propositions, representing tasks, are written in $\msf{sans}$
$\msf{serif}$ fonts. Notice that we do not pose any restrictions on
how tasks are structured but which data they access (as specified by
predicate $uses$). Therefore, in practical terms, process
tasks can play the role of atomic actions as well as automated complex
programs, external \textsc{soa} services or tasks involving human
activities (called human tasks in the \bpm literature).

\begin{compactitem}
\item $\msf{interview}$ is a constraint forcing $\msf{interview}$ to
  be the first task of the process;
\item
  $\Diamond \msf{optIn} \lor \Diamond \msf{optOut} \land \neg
  (\Diamond \msf{optIn} \land \Diamond \msf{optOut})$
  means that eventually the student has to decide whether or not
  giving the consent to access his/her university data;
\item $\neg \msf{getExams} \Until \msf{optIn}$ expresses that activity
  $\msf{getExams}$, which accesses the students exam list, cannot be
  performed unless $\msf{optIn}$ has been previously executed;
\item
  $\neg \msf{findJobs} \Until (\msf{getExams} \lor
  \msf{getExperiences})$
  means that it is not possible for the company to find jobs if it
  could not acquire any of the student's data before;
\item $\Diamond \msf{findJobs}$ indicates that eventually
  $\msf{findJob}$ must be performed;
\item $\msf{findJobs} \ra \Next \msf{proposeJob}$ forces task
  $\msf{proposeJob}$ to be executed right after $\msf{findJobs}$;
\item $\Diamond (\msf{chooseJob} \lor \msf{abort})$ expresses
  that eventually either a job has to be chosen by the student or the
  process is aborted.
\end{compactitem}

\end{example}

We remark that the declarative approach leaves, in general, infinite
ways of satisfying the constraints. Our processes do not claim to be
complete, but rather to provide an easy and straightforward intuition
of both the power of the declarative approach and the processes. As a
consequence, there could be executions formally satisfying the
constraints which do not meet our informal intuition of the processes.


% Indeed, while some tasks has to be
% executed in a specific order, some others can be executed in parallel,
% such as $\msf{getExams}$ and $\msf{getExperiences}$, or not executed
% at all, e.g., $\msf{getExams}$ when the students opts-out its consent
% to access university data.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


\endinput

==> 4bis-results.tex <==
\section{Results}

Both offline and runtime verification techniques we use to carry out
the three policies verification described in the previous Section are
automata-based, meaning that reasoning is solved by manipulating
finite-state automata. Indeed, a propositional \LTL formula $\phi$ on
finite-traces can be associated with a finite-state automaton $A$
which recognizes exactly the (finite) traces that make $\phi$ true. We
denote by $L(A)$ the set of traces, i.e., the language, recognized by
$A$.
%%
\begin{lemma}[\cite{Vardi95}, \cite{DeGiacomoV13}, \cite{DeGiacomoMGMM14}]
  Let $\P$ a set of propositional symbols, $\phi$ a \LTL
  (finite-trace) formula over $\P$ and $\pi$ a trace. Then there
  exists an automaton $A_{\phi}$ such that $\pi \models \phi$ iff
  $\pi \in L(A_{\phi})$.
\end{lemma}
\begin{proofsk}
  % As shown in \cite{Vardi95} and \cite{DeGiacomoV13}, \LTL on finite
  % traces is less expressive than regular expressions (\RE) (to be
  % precise, \LTL is equivalent to star-free regular expressions
  % \cite{McNaughton}). Being well-known the correspondence between \RE
  % and finite-state automaton, in principle $\phi$ can be translated
  % into a \RE $\rho$ and then the automaton for $\rho$ can be
  % built. Unfortunately, such a translation introduce a nonelementary
  % complexity in the length of the formula, i.e., an unbounded
  % stack of exponentials, due to the fact that negation in \LTL
  % corresponds to complementation in \RE, which, in turn, require an
  % exponential step.
  In \cite{DeGiacomoMGMM14}, a direct algorithm for building a
  finite-state automaton $A_{\phi}$ from $\phi$ is shown. The algorithm is
  based on the traditional translation in \cite{DeGiacomoV13} and
  \cite{Vardi95} which first builds the alternating automaton for
  $\phi$ and then translates the alternating automaton into a
  finite-state automaton.  The algorithm runs in exponential number of
  steps in the size of $\phi$, and generates an automaton whose set of
  states is at most exponential in the size of $\phi$.
\end{proofsk}

An automaton for a \LTL formula over $\P$ is a finite-state machine
whose edges are labeled with propositional interpretations for symbols
in $\P$. In our case, however, since formulas are used to represent
processes, $\P$ to represent tasks, and the constraint expressing that
only one task is performed at a time is implicitly assumed (see
Section \ref{sec:purpose}), interpretation on edges assigns $true$ to
only one symbol (task) in $\P$ and $false$ to the others.


% \begin{lemma}[\cite{DeGiacomoV13}, \cite{SistlaClarke1985}]
% Satisfiability, validity and logical implication of \LTL formulas on
% finite traces are \textsc{pspace}-complete.
% \end{lemma}
% \begin{proofsk}
%   \textsc{pspace} membership follows from the fact that satisfiability
%   of \LTL on finite traces can be reduced to that on infinite traces,
%   which, in turn, is \textsc{pspace}-complete
%   \cite{SistlaClarke1985}. \textsc{pspace}-hardness is obtained by
%   adapting the original proof for \LTL on infinite traces
%   (\cite{SistlaClarke1985}) to finite traces.
% \end{proofsk}


Once we have the finite-state automaton $A_{\phi}$, satisfiability of
$\phi$ reduces to check whether exists a path to a final state in
$A_{\phi}$. This problem is called \emph{nonemptiness} of $A_{\phi}$
and it is \textsc{pspace}-complete.

\begin{lemma}[\cite{DeGiacomoV13}, \cite{SistlaClarke1985}]
Satisfiability, validity and logical implication of \LTL formulas on
finite traces are \textsc{pspace}-complete.
\end{lemma}
\begin{proofsk}
  \textsc{pspace} membership follows from the fact that satisfiability
  of \LTL on finite traces can be reduced to that on infinite traces,
  which, in turn, is \textsc{pspace}-complete
  \cite{SistlaClarke1985}. \textsc{pspace}-hardness is obtained by
  adapting the original proof for \LTL on infinite traces
  (\cite{SistlaClarke1985}) to finite traces. Validity of $\phi$
  reduces to checking satisfiability of $\neg \phi$ and logical
  implication $\phi_1 \models \phi_2$ reduces to satiability
  of $\phi_1 \land \neg \phi_2$.
\end{proofsk}


Given two \LTL formulas $\phi_1$ and $\phi_2$, checking if $\phi_1$ is
a sub-purpose of $\phi_2$ means verifying whether
$\phi_2 \models \Diamond \phi_1$. From the above lemmas it follows
immediately that:

\begin{theorem}
  The \emph{offline sub-purpose verification} problem is
  \textsc{pspace}-complete.
\end{theorem}


We now move to the \emph{offline process completion verification} and
\emph{runtime policies verification}.  Differently from the
\emph{offline sub-purpose verification}, where only the
(propositional) specification of processes is analyzed, now also \sod,
\bod and \rbac policies are taken into account, which require a
first-order reasoning on the database instance and on the temporal
execution of the system. Furthermore, the temporal reasoning on
$\msf{p}$, dealing with the sequence of tasks to be performed, cannot
be decoupled from the first-order reasoning on the database instance
storing the policies, because the presence of \sod and \bod contraints
keeps this two aspects connected.

In order to solve the problem, we follow the approach in
\cite{DeMasellisMM14}, where the traditional propositional \declare is
extended to support \emph{data-aware} constraints. Indeed, the main
limitation of \declare is the lack of data support, as only atomic
activities are considered: the proposed extension aims at overcome
this difficulty by attaching a payload to activities and augmenting
the contraints queries on the payload itself and the database. 
%%
The setting in \cite{DeMasellisMM14} is very similar to ours: data are
stored in a database and events occurring in the system change such
data. In this setting, the interest is not only in checking sequence
of events, but also in verifying that data complies with (or are
modified according to) specific contraints. Thus, traditional \declare
constraints are equipped with a first-order syntax with temporal
operators, giving rise to a first-orer temporal logic.
%%
Roughly speaking, when a new event, namely, a new request, is
performed to the system, we would like to verify a condition on the
database instance, which represent the privacy policies.  Therefore,
traditional \LTL contraints composing our processes are automatically
transformed in the conjunction of two first-order formulas intuitively
representing a query on the database: the first one is on the dynamic
part of the database and selects payload of the request and the second
one verifies that the payload meet the policies. As an example,
consider the propositional \LTL contraint $\Diamond \msf{findJobs}$ of
process $\msf{jobHunting}$. Its first-order translation is:
\[ \begin{array}{c}
\Diamond \exists sub, do.(request(pid, sub, \msf{findJobs}, do,
\msf{jobHunting}) \land \\\\
\forall act,obj. uses(act, \msf{findJobs}, obj) \ra \\
(accessibleFor(do, obj, \msf{jobHunting}) \land auth(sub, act,
obj)))
\end{array}
\]
Intuitively, the first conjunct verifies that the current request is
for task $\msf{findJob}$ and the second verifies that $sub$ has the
rights to access all data $\msf{findJob}$ manipulates.

Our whole processes can then be automatically translated following the
consideration above. The reason why we decided to first express the
contraints in propositional form and then translating them instead of
directly having them in a first-order syntax is merely
practical. Usually, processes are specified by non-technical people,
with the help of graphical tools such as the ones made available for
traditional \declare, which cannot be overwhelmed by the formal
details. Notably, our approach allows to decouple the specification of
the process from their actual implementation in our system, and
furthermore, the translation can be performed automatically.

We now show an excerpt of the translated formula
$\Psi_{\msf{jobHunting}}(id)$ for the $\msf{jobHunting}$ process.
% The solution is explained with
% the help of our running example. Let us assume $I_{st}$ expresses some
% generic \rbac policies over data owner $\msf{do}$ and we want to
% verify the offline completion of $\msf{jobHunting}$, which contains
% \sod and \bod contraints. We consider a generic process execution with
% identifier $\msf{id}$ and build a first-order temporal
% formula $\Psi$ which essentially incorporates \rbac, \sod, \bod and
% purpose-based contraints in a unique formula.
%%
   \[ \begin{array}{c}
        \exists sub1, sub2.\\
        ( \exists do.(request(id, sub1, \msf{interview}, do,
        \msf{jobHunting}) \land \\
\forall act,obj. uses(act, \msf{interview}, obj) \ra \\
accessibleFor(do, obj, \msf{jobHunting}) \land auth(sub1, act,
        obj)) \land \\

        \ldots \\
        
 \neg \exists sub,do.request(\msf{id}, sub, \msf{getExams}, do,
         \msf{jobHunting}) 
% \land \\ (\exists sub. uses(act, \msf{getExams}, obj) \ra \\
% (accessibleFor(\msf{do}, obj, \msf{jobHunting}) \land auth(sub, act,
%         obj))) \land
        \\ \Until \\

\exists sub,do.(request(id, sub, \msf{optIn}, do,
\msf{jobHunting}) \land \\
\forall act,obj. uses(act, \msf{optIn}, obj) \ra \\
(accessibleFor(do, obj, \msf{jobHunting}) \land auth(sub, act,
obj))) \land \\

        \ldots \\
        \Diamond (\exists do.(request(\msf{id}, sub2, \msf{findJobs}, do,
        \msf{jobHunting}) \land \\
        \forall act,obj. uses(act, \msf{findJobs}, obj) \ra \\
        accessibleFor(do, obj, \msf{jobHunting}) \land auth(sub2, act,
        obj)) \land \\

\ldots \\
\land sub1 \not = sub2)
\end{array} \]
%%
Subjects are \emph{locally} quantified when they are not
involved in any \sod and \bod contraints, namely quantification does
not involves temporal operators in its scope. To the contrary, when
such contraints are present, then the quantification for subjects is
brought at the beginning of the formula and includes, in its sope,
temporal operators.
%%
Notice also that variable $id$ is \emph{free}, and has to be
substituted with an actual value in order for the formula to be
evaluated.



% In this case we say that the quantification is
% \emph{across-state} and involves a hard and costly kind of temporal
% reasoning.
%%
% Formula $\Psi$ represents, in a first-order syntax, all \rbac, \sod,
% and \bod contraints to be fulfilled by a generic process execution
% $\msf{id}$. If there exists a finite trace $\Pi|_{\msf{id}}$ that
% satisfies $\Psi$, then the offline process completion verification has
% a positive solution.
%%
Unfortunately, first-order temporal logic is, in general, undecidable
\cite{BauerKV13}, but in our case, two important considerations are to
be made. The first one concerns the static part of the database: since
it stores the \rbac policies, it is reasonable assuming \emph{complete
  information}. Indeed, once policies are specified, everything that
is not explicitly allowed must be forbidden. This assumptions are of
fundamental importance because provides for considering elements that
are in the current active domain $adom(I_{st})$ only.
%%
The second one is about the dynamic part: the same considerations
cannot be done, as new process ids are continuously generated
throughout the system execution, and cannot be predicted nor
bounded. As a consequence, quantifications of variables of sort
$Processes$ spans over the infinite domain $\Delta_{proc}$.

In what follows we separately tackle the issue of the infinite
$\Delta_{proc}$ domain for the \emph{offline process
  completion verification} and \emph{runtime policies verification} to
achieve decidability.




\subsection{Offline process completion verification}

Let us assume our $\msf{jobHunting}$ process along with \sod and \bod
contraints and a database instance $I_{st}$ specifying \rbac and
purpose-based policies for a generic data owner $\msf{do}$. We would
like to check if there is a way to successfully execute
$\msf{jobHunting}$ given the policies. We build a formula
$\Upsilon_{jobHunting}$ which is satisfiable iff $\msf{jobHunting}$
process can be successfully completed given the policies in $I_{st}$.

Formula $\Upsilon_{jobHunting}$ is obtaining by specializing formula
$\Psi_{jobHunting}(id)$. First of all, since we are interested in a
generic process instance $\msf{id}$ we substitute the value $\msf{id}$
to the free variable $id$ in $\Psi_{jobHunting}[\msf{id}/id]$. We also
have to enforce that the privacy policies in $I_{st}$ does not change
during the execution. We observe that a database instance $I_{st}$,
given the complete information assumption, can be seen as a
logic formula, which is the conjunction of all positive facts
$R(d_1 \ldots d_n)$ when $(d_1 \ldots d_n) \in R^I$ and the
conjunction of all negative facts $\neg R(d_1 \ldots d_n)$ when
$(d_1 \ldots d_n) \not \in R^I$. Le us denote by $I_{st}$ such a
formula with notational abuse. Then, forcing the static part of the
database to be fixed means adding the constraint $\Box I_{st}$ to
$\Psi_{jobHuting}[\msf{id}/id]$.


\begin{lemma}
  Let $\msf{proc}$ be a process with possibly \sod and \bod contraints
  and let $I_{st}$ specify a set of \rbac policies. Then formula
  satisfiability of $\Psi_{proc}[\msf{id}/id] \land \Box I_{st}$ is
  decidable in exponential space in the length of the formula.
\end{lemma}
%%
\begin{proofsk}
  Formula $\Psi_{proc}[\msf{id}/id] \land \Box I_{st}$ is ground and,
  given the complete information assumption, \emph{all its quantifiers
    span over finite sorts} contained in $adom(I_{st})$. So it can be
  \emph{propositionalized} by simply expanding each universally
  quantified variable on a specific sort with the conjunction of the
  (finite) assignments for that sort. Analogously, existential
  quantifiers are expanded by the disjunction of all assignments. The
  automata for the propositionalized formula can then be build and its
  nonemptiness can be checked.
%%
The propositionalization of a first-order formula generates a new
formula which length can be exponential in the size of the active
domain $adom(I_{st})$. The automaton construction then introduces
another exponential blowup. However, there are symbolic techniques that
build the automaton for a first-order formula with bounded domain in
exponential size in the length of the formula
\cite{DeMasellisS13}. To be more precise, the overall construction requires is
exponential space in the number of across-state variables, i.e., those
required by \sod and \bod contraints.
\end{proofsk}


\begin{theorem}
  Let $\msf{proc}$ be a process with possibly \sod and \bod contraints
  and let $I_{st}$ specify a set of \rbac policies. Then checking
  whether $\msf{proc}$ can be successfully competed given the policies
  can be solved in exponential space in the size of $\msf{proc}$.
\end{theorem}

\begin{proofsk}
  Process $\msf{proc}$ can successfully complete iff
  $\Psi_{proc}[\msf{id}/id] \land \Box I_{st}$ is satisfiable. The
  above formula is satisfiable iff there exists a finite trace
  $\Pi=I_1, \ldots, I_n$ which complies with the contraints of
  $\msf{proc}$ expressed by $\Psi_{proc}[\msf{id}/id]$ assuming that
  the policies does not change, that is formalized by $\Box
  I_{st}$. Considering the above lemma, we get the conclusion.
\end{proofsk}




\subsection{Runtime policies verification}




%%
Formula $\Psi$, however, fixes the process id to a generic one, hence
all its quantifiers spans over the finite domain
$adom(I_{st})$. Moreover, it does not contain any free variable. It
turns then out that $\Psi$ can be transformed into propositional
formula by simply expanding each universally quantified variable on a
specific sort with the conjunction of the (finite) assignments for
that sort (taking values from $adom(I_{st})$). Analogously,
existential quantifiers are expanded by the disjunction of all
assignments.  \todo[inline]{Mandare come riferimento ICSOC13 e
  ICSSP14.}
%%
%%
Also a database instance $I$, given the complete information
assumption, can be propositionalized. Indeed, it can be seen as a
logic formula, which is the conjunction of all positive facts
$R(d_1 \ldots d_n)$ when $(d_1 \ldots d_n) \in R^I$ and the
conjunction of all negative facts $\neg R(d_1 \ldots d_n)$ when
$(d_1 \ldots d_n) \not \in R^I$.
%%
For the sake of readability, we keep the same notation for first-order
formulas and their propositionalized version, as well as database instances.

Formula $\Psi$ (propositionalized) can hence be evaluated over a
(propositionalized) trace $\Pi=I_1, I_2, I_3, \ldots$. As usual,
instance $I_i$ provides a truth assignments for propositional symbols
in $\Psi$ at time instant $i$.
%%
Nonemptiness of automaton $A(\Psi)$ would answer to whether there
exists a trace $\Pi$ satisfying $\Psi$. Our problem, instead, is to
verify if the specific policies in $I_{st}$ can lead to the
satisfaction of $\Psi$. Formally, what we are looking for is the
existence of a trace
$\Pi = I_{st}\cup I^1_{dy}, I_{st}\cup I^2_{dy}, I_{st}\cup I^3_{dy},
\ldots$ where the static part does not change. To force this problem 




















%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

\endinput


% The distinction between \rbac and \sod and \bod along with
% the technical difficulties in incorporating the latter, is now
% explained more in detail. \rbac policies do not depend on a specific
% process execution and, more importantly, do not change during
% execution, being fixed once and for all.


% Hence, when no \sod and \bod
% are considered, \emph{offline process completion verification} can be
% addressed as follows. We first generate the propositional automaton
% $A_{\msf{p}}$ for process $\msf{p}$. Then, we trim $A_{\msf{p}}$ by
% dropping the edges labeled with tasks which cannot be executed due to
% current policies (recall that each edge is labeled with a single task
% only). Finally, we check the nonemptiness of the trimmed automaton.
% The challenging part is attest when a task $\msf{t}$ can actually be
% performed. In logical terms, this translates into:
% \[
% \begin{array}{c}
% I_{st} \models \exists sub \; \forall act, obj.uses(act, \msf{t}, obj)  \ra \\
% (accessibleFor(\msf{do}, obj, \msf{p}) \land auth(sub, act, obj))
%   \end{array}
%   \]
% i.e., if there exists a subject $sub$ having the privileges to access
% all data task $\msf{t}$ manipulates for purpose $\msf{p}$.
% %%
% It is easy to see that checking the above formula is decidable, and
% actually reduces to test if the above query over $I_{st}$ is not empty:

% \todo[inline]{completare la query}

==> 6-conclusion.tex <==
%!TEX root = ./main.tex

\section{Conclusions and Future work}
\label{sec:concl}

We have presented a declarative framework based on first-order \LTL to
specify and enforce purpose-aware policies.  The basic building blocks
of purpose-aware policies are data- and rule-centric policies,
expressed in (fragments of) first-order logic, together with workflows
augmented by authorization constraints, expressed in \LTL following
the declarative approach to business process specification
in~\cite{WestergaardM11,AalstPS09}.  A first-order \LTL formula is
then defined from the \LTL expression describing the workflow
associated to a purpose in a policy by taking into the first-order
formulae expressing data- and rule-centric policies.  Such a
first-order temporal formula is used to build an automaton for the
run-time monitoring and enforcement of the purpose-aware policy.  By
reusing results available in the literature about the satisfiability
of first-order \LTL (over finite traces), we have been able to show
that answering, at run-time, a request requires exponential time in
the number of authorization constraints in the purpose-aware policy
(Theorem~\ref{thm:main}).  This is as expected as answering requests
under purpose-aware policies in our framework requires to solve the
Workflow Satisfiability Problem~\cite{crampton}, which is known to be
NP-hard in the presence of one \sod constraint~\cite{wang-li}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% In this paper we have introduced a formal framework for:
%% \begin{inparaenum}[(i)]\item the
%%   representation, \item offline verification and \item runtime
%%   monitoring
%% \end{inparaenum}
%% of purpose-aware, \rbac, \sod and \bod privacy policies by means of
%% decidable methods. The approach is based on the intuitive notion of
%% purpose as the specific objective (goal) for which data are used for,
%% together with the sequence of tasks needed to realize it, represented
%% by means of declarative (business) workflows. The formal framework and
%% techniques exploit and customize the solid formal basis of
%% representation, verification and monitoring of (business) workflows
%% based by using first-order linear time temporal logic,
%% thus expanding the impact of formal methods techniques into data
%% privacy.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
As future work, we envisage to implement a run-time monitor for
purpose-aware policies on top of a workflow management system (e.g.,
that in~\cite{WestergaardM11}) and a library for manipulating automata
(e.g., the one in~\cite{DeGiacomoMGMM14}) and to study if and how to
extend our framework to consider \emph{inter-workflow constraints},
i.e.\ authorization constraints involving different workflow
instances.
%% Also, we plan to extend \declare and access control tools to
%% incorporate the proposed techniques.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

\endinput

